Flash-KMeans: Fast and Memory-Efficient Exact K-Means

$k$-means has historically been positioned primarily as an offline processing primitive, typically used for dataset organization or embedding preprocessing rather than as a first-class component in online systems. In this work, we revisit this classical algorithm under the lens of modern AI system design and enable $k$-means as an online primitive. We point out that existing GPU implementations of $k$-means remain fundamentally bottlenecked by low-level system constraints rather than theoretical algorithmic complexity. Specifically, the assignment stage suffers from a severe IO bottleneck due to the massive explicit materialization of the $N \times K$ distance matrix in High Bandwidth Memory (HBM). Simultaneously, the centroid update stage is heavily penalized by hardware-level atomic write contention caused by irregular, scatter-style token aggregations. To bridge this performance gap, we propose flash-kmeans, an IO-aware and contention-free $k$-means implementation for modern GPU workloads. Flash-kmeans introduces two core kernel-level innovations: (1) FlashAssign, which fuses distance computation with an online argmin to completely bypass intermediate memory materialization; (2) sort-inverse update, which explicitly constructs an inverse mapping to transform high-contention atomic scatters into high-bandwidth, segment-level localized reductions. Furthermore, we integrate algorithm-system co-designs, including chunked-stream overlap and cache-aware compile heuristics, to ensure practical deployability. Extensive evaluations on NVIDIA H200 GPUs demonstrate that flash-kmeans achieves up to 17.9$\times$ end-to-end speedup over best baselines, while outperforming industry-standard libraries like cuML and FAISS by 33$\times$ and over 200$\times$, respectively. Our code is open-sourced at https://github.com/svg-project/flash-kmeans.

==> text/1_Introduction_v0.tex <==
\section{Introduction}

\kmeans is one of the most classical and widely used clustering algorithms, and has long been treated as a mature, general-purpose component. 
In traditional settings, \kmeans typically appears as part of offline data processing pipelines, and most optimizations focus on the algorithmic level, such as faster convergence, fewer distance evaluations, or better approximations. 
Although these algorithmic improvements can reduce the computation cost, many of them do not translate into real end-to-end speedups on modern GPUs. 
One main reason is that they primarily target FLOP reduction\haocheng{Not compatible with modern design principle of GPUs - Compute / Matmul is cheap, while frequent fragmented operations leads to huge overhead}, which does not necessarily correlate with wall-clock time, and often overlooks overheads from memory access and data movement.
As a result, despite its simple mathematical form, the performance of \kmeans can be constrained by low-level implementation \haocheng{the real end-to-end latency is inconsistent with their FLOPs savings}.

This performance gap caused by implementation-level factors is significantly amplified in modern AI workloads. That is because \kmeans usage is undergoing a clear paradigm shift, evolving from an offline analytics tool into a high-frequency operator within training and inference pipelines. 
This shift manifests in three dimensions: (1) execution moves from CPUs to GPUs, and datatypes move from FP32 and FP64 to FP16, BF16, and even lower-bit formats, which creates clear potential to exploit hardware accelerators; (2) usage moves from offline to online invocation, making low latency per invocation essential; (3) computation\haocheng{workload} moves to longer sequences and larger batches, making throughput and scalability crucial requirements. \haocheng{Why this appears both in Section 1 and 3}
These changes move the bottlenecks beyond algorithmic complexity toward system constraints, including GPU data movement and bandwidth, write-side atomic contention, and compilation and deployment overheads under dynamic shapes. This motivates a fresh look at efficient \kmeans implementations for modern GPU workloads.

\haocheng{Before introducing these challenges, we need to first define the \kmeans workload. For example, we need to say explicitly that, it contains two stages. One is assignment stage, one is update stage.}


% (3) \textbf{System overheads matter in real deployments.}
% In large-scale or memory-constrained settings, K-means often requires chunked execution with host-to-device communication. Moreover, dynamic shapes and cross-hardware deployment amplify compilation and configuration tuning overheads. These costs do not change asymptotic algorithmic complexity, but directly impact time-to-first-run and end-to-end latency, limiting practical usability in online workloads.

We begin by profiling a standard \kmeans implementation and find that its end-to-end performance on modern GPUs is often limited by kernel-level and system-level overhead. Concretely, this performance gap arises from three primary challenges:

\begin{enumerate}
    \item IO-bound assignment: for a \kmeans iteration with $N$ points, feature dimension $d$, and $K$ clusters, the assignment step compares every point against every centroid, with a compute cost of $O(NKd)$. 
    \haocheng{This sentence is strange. Maybe: Consider a workload consisting of $N$ data points in $d$-dimensional space. We perform \kmeans clustering with $K$ clusters. In each iteration, the assignment step compares every point with all $K$ centroids, resulting in a computational cost of $O(NKd)$.}
    Standard implementation first computes distances and then applies $\arg\min$, which materializes a distance matrix $D\in\mathbb{R}^{N\times K}$.
    This introduces a short-lived but massive intermediate: writing $D$ to HBM and reading it back incurs huge memory traffic. 
    Under a representative setting with $N=\fixme{}, K=\fixme{}, d=\fixme{}$, we observe that the distance computation itself takes about \fixme{}, whereas the memory time dominated by materializing and consuming $D$ takes about \fixme{}.
    \item Atomic write contention: \kmeans centroid update stage is a pure aggregation \haocheng{Need to define in advance that this update stage is simply an average operation over specific indices} that should ideally approach the bandwidth ceiling of regular reductions. However, standard implementation typically performs scatter-style updates: each point $x_i$ atomically accumulates into the sum buffer $s_{a_i}$ and count buffer $n_{a_i}$ according to its cluster id $a_i$. 
    As a result, many threads concurrently update the same centroid or a few hot centroids, causing severe atomic contention and serialization.
    On a \fixme{} GPU, we measure only \fixme{}~GB/s effective bandwidth for this stage, far below the achievable bandwidth of regular reductions or streaming reads and writes on the same hardware.
    \item System-level limits: beyond the kernel-level bottlenecks, \kmeans is also constrained by other system-level factors in real deployments. 
    When the input cannot reside entirely on the GPU, chunk-wise execution introduces host-to-device communication and synchronization overheads. 
    In addition, modern workloads often have dynamic shapes, which amplify compilation and configuration tuning costs, increasing \ttfr and hurting practical usability. 
\end{enumerate}

% Beyond the kernel-level bottlenecks, \kmeans is also constrained by other system-level factors in real deployments. 
% When the input cannot reside entirely on the GPU, chunk-wise execution introduces host-to-device communication and synchronization overheads. 
% In addition, modern workloads often have dynamic shapes, which amplify compilation and configuration tuning costs, increasing \ttfr and hurting practical usability. 
% As a result, algorithm-system co-design is needed to enable practical real-world deployment.

% To address the three bottlenecks above, we propose \method, an efficient \kmeans implementation for modern GPU workloads. \Method does not change the mathematical form of standard Lloyd K-means and does not introduce approximation. Instead, it is designed around the three dominant sources of overhead in standard implementations: the IO bottleneck from distance materialization in assignment, the write-path contention from atomic adds in centroid update, and the system overheads introduced by large-scale data movement and dynamic shapes in real deployments. 
% In this sense, the goal of Flash-KMeans is not to further reduce theoretical FLOPs, but to make K-means execution better match the data path and runtime characteristics of modern GPUs.

To bridge this performance gap, we propose \method, an efficient implementation of \kmeans for modern GPU workloads. 
\Method does not change the mathematical form of the standard Lloyd \kmeans. 
Instead, it systematically restructures the assignment stage, the centroid update stage, and the system execution path around the three bottlenecks discussed above.

Concretely, these three bottlenecks are addressed by the three key techniques in \method. To avoid distance materialization in assignment, we introduce \textit{\FA}, which replaces the standard two-stage pipeline of first materializing distances and then reducing them with a streaming distance computation and the online argmin procedure, thereby avoiding the explicit construction of the $N\times K$ intermediate and reducing the round trips of HBM. 
To reduce atomic contention in centroid update, we introduce \textit{\siu}, which first sorts assignments by cluster id and then performs aggregation in the sorted logical order, rewriting per-token atomic scatter into more regular segment-level merging. 
To address the system overheads from large-scale execution and dynamic deployment, we further introduce a set of \textit{algorithm-system co-design} optimizations, including \cso and \compileheuristic, which respectively hide communication overhead and reduce configuration tuning cost. 
Together, these three techniques enable \method to remain mathematically equivalent to standard Lloyd \kmeans while delivering more stable end-to-end speedups on modern GPU workloads.

We prototype \method with customized GPU kernels and evaluate it systematically on NVIDIA H100. 
We first compare end-to-end latency across a sweep of the number of points $N$, the number of clusters $K$, the feature dimension $d$, and batch size $B$\haocheng{Simply mention multiple workload here is OK}. \method achieves the best performance across three representative workload regimes, outperforming the strongest baseline by up to \fixme{}$\times$ and by \fixme{}$\times$ on average. \haocheng{We should mention this after kernel-level breakdown right?}
A kernel-level breakdown further shows that \FA speeds up the assignment kernel by up to \fixme{}$\times$, and \siu speeds up the centroid update kernel by up to \fixme{}$\times$. 
Beyond kernel-level acceleration, we also evaluate the two algorithm-system co-design optimizations. In the large-scale setting, \cso further reduces end-to-end runtime by \fixme{}\% through overlapping communication with computation. 
Under dynamic shapes and cross-hardware deployment, the \compileheuristic matches the best tuned configuration within \fixme{}\% performance difference while reducing compile and tuning overhead by \fixme{}$\times$. 
These results show that \method is not only efficient at the kernel level, but also delivers stable and deployable end-to-end acceleration for modern GPU workloads.


==> text/3_Motivation_v0.tex <==
\section{Motivation}

\subsection{K-Means Workloads are Undergoing a Paradigm Shift}
\lblsect{motivation-paradigm-shift}

\kmeans workloads are shifting from ``offline data processing'' to ``online primitive'' in AI systems. 
In traditional settings, \kmeans is typically executed as an offline analytics or preprocessing step, including one-shot clustering in classical data mining pipelines and codebook construction in conventional computer vision workflows.
These workloads are largely CPU-centric, assume data resident in host memory, rely primarily on FP32 or FP64 datatypes, exhibit relatively stable input shapes, and are generally insensitive to \ttfr costs such as compilation and configuration search.
\fixme{Add more concrete examples}

Compared with the traditional regime, the emerging \kmeans workload has three defining characteristics: (1) execution shifts from CPUs to GPUs, and datatypes move from FP32 and FP64 to FP16, BF16, and even lower bit formats, which creates clear potential to exploit hardware accelerators; 
(2) usage shifts from offline to online, which makes low latency per invocation essential; 
(3) computation shifts from small batches to large batches.
These patterns arise in \KVc quantization and vector quantization style codebook updates, where centroids are refreshed repeatedly during training or inference. They also appear in sparse attention, token grouping, and routing, where clustering is used to form structured sparsity or grouped computation. In attention based models, the number of tokens and attention heads further amplifies this effect, making the associated online K means calls naturally large batch.
As a result, the optimization target extends beyond offline throughput to system level criteria such as stable performance under dynamic shapes and heterogeneous GPUs, low \ttfr, and tight integration with input output and memory constraints.

\subsection{Standard K-Means Implementation is IO-Bottlenecked}
\lblsect{motivation-io}

\fixme{talk about centroid update part}

\mypara{Euclidean \kmeans via Lloyd's iterations.}
Given data points $X\in\mathbb{R}^{N\times d}$ and centroids $C\in\mathbb{R}^{K\times d}$, Euclidean \kmeans minimizes
\begin{equation}
\min_{a\in\{1,\dots,K\}^N,\; C}\;\sum_{i=1}^{N}\left\lVert x_i-c_{a_i}\right\rVert_2^2 .
\end{equation}
Lloyd's algorithm alternates between (i) an assignment step \haocheng{Better to also say $D\in \mathbb{R}^{N\times K}$}
\begin{equation}
D_{ik}=\left\lVert x_i-c_k\right\rVert_2^2,\qquad a_i=\arg\min_{k} D_{ik},
\end{equation}
and (ii) a centroid update step
\begin{equation}
n_k=\sum_{i=1}^{N}\mathbb{I}[a_i=k],\quad
s_k=\sum_{i=1}^{N}\mathbb{I}[a_i=k]\,x_i,\quad
c_k\leftarrow \frac{s_k}{n_k}.
\end{equation}
In practice, the squared distance is often expanded as
\begin{equation}
\label{eq:dist_expand}
\left\lVert x_i-c_k\right\rVert_2^2=\lVert x_i\rVert_2^2+\lVert c_k\rVert_2^2-2x_i^\top c_k,
\end{equation}
which enables the reuse of norms and maps the computation to high-throughput matrix multiplications.

\mypara{Standard Lloyd's iteration implementation.\haocheng{For Assignment Step?}}
Many existing libraries follow a direct and general implementation that materializes large intermediate tensors. \haocheng{Which tensor, D?}
Algorithm~\ref{alg:standard_kmeans} summarizes a typical iteration: it first computes and writes a blockwise distance matrix to HBM,
then reads it back for row-wise reduction to obtain assignments, and finally aggregates points per cluster to update centroids.

\begin{algorithm}[h]
\caption{Standard \kmeans implementation (one iteration)\haocheng{Need to rewrite this algorithm}}
\label{alg:standard_kmeans}
\KwIn{$X\in\mathbb{R}^{N\times d}$, $C\in\mathbb{R}^{K\times d}$ resident in HBM}
\BlankLine
\textbf{Distance:} Load blocks of $X$ and $C$ from HBM, compute $D\in\mathbb{R}^{N\times K}$ (via Eq.~\eqref{eq:dist_expand}), and write $D$ to HBM\;
\textbf{Assign:} Read $D$ from HBM, compute $a_i=\arg\min_k D_{ik}$ for each $i$, and write $a\in\{1,\dots,K\}^N$ to HBM\;
\textbf{Update:} Read $X$ and $a$ from HBM, accumulate $(s_k,n_k)$ for all $k$ (e.g., scatter-add or indicator-based aggregation), write $s\in\mathbb{R}^{K\times d}$ and $n\in\mathbb{R}^{K}$ to HBM\;
\textbf{Normalize:} Compute $C\leftarrow s \oslash n$ and write updated centroids $C$ to HBM\;
\end{algorithm}

\mypara{Why the standard implementation is IO bound.}
The key inefficiency is the explicit materialization of the distance matrix $D\in\mathbb{R}^{N\times K}$.
$D$ is a short-lived intermediate that is written to HBM in the distance kernel and immediately read back in the assignment kernel.
This incurs at least $\Theta(NK)$ writes plus $\Theta(NK)$ reads per iteration, dominating the total memory traffic when $N$ and $K$ are large.
In contrast, other tensors are comparatively smaller: reading $X$ and $C$ costs $\Theta(Nd+Kd)$, writing assignments costs $\Theta(N)$,
and writing cluster statistics costs $\Theta(Kd+K)$.
As a result, even if the distance computation uses high-throughput primitives, the end-to-end iteration is typically bandwidth limited by
the $2\cdot\Theta(NK)$ HBM round trips for $D$.
This observation motivates IO-aware reorganizations that compute distances in tiles and reduce them on chip immediately, thereby avoiding
materializing the full $N\times K$ intermediate in HBM.


\subsection{Other System Constraints in GPU Workloads.}

Beyond the IO bottleneck discussed above, \kmeans faces a new set of system constraints in modern GPU workloads. First, \kmeans is invoked frequently and at large batch sizes in AI pipelines, while sharing GPU memory with activations, \KVc, and other operators. 
As a result, device memory quickly becomes a practical bottleneck. Chunking reduces peak memory usage, but it can introduce frequent CPU to GPU communication and synchronization, which again limits end to end throughput.
Second, GPU hardware differs substantially in compute capability, memory bandwidth, cache capacity, and register resources, so a kernel configuration that works well on one device may not remain efficient on another. This makes cross hardware performance robustness an important requirement rather than a secondary concern. 
Finally, real pipelines often have dynamic shapes, with changing numbers of points, clusters, and feature dimensions. If an implementation relies heavily on shape specialization and full auto-tuning, shape changes can trigger frequent recompilation and configuration search, increasing \ttfr and reducing practical usability. 
These constraints directly motivate our \cso design and \compileheuristic in \sects{co-design}.

==> text/5_Implementation.tex <==
\section{Implementation}
